Improved motif-scaffolding with SE(3) flow matching

Protein design often begins with the knowledge of a desired function from a motif which motif-scaffolding aims to construct a functional protein around. Recently, generative models have achieved breakthrough success in designing scaffolds for a range of motifs. However, generated scaffolds tend to lack structural diversity, which can hinder success in wet-lab validation. In this work, we extend FrameFlow, an SE(3) flow matching model for protein backbone generation, to perform motif-scaffolding with two complementary approaches. The first is motif amortization, in which FrameFlow is trained with the motif as input using a data augmentation strategy. The second is motif guidance, which performs scaffolding using an estimate of the conditional score from FrameFlow without additional training. On a benchmark of 24 biologically meaningful motifs, we show our method achieves 2.5 times more designable and unique motif-scaffolds compared to state-of-the-art. Code: https://github.com/microsoft/protein-frame-flow

==> content/experiments/unconditional.tex <==

We present backbone generation results of the unconditional FrameFlow model used in FrameFlow-guidance.
We do not perform an in-depth analysis since this task is not the focus of our work.
Characterizing the backbone generation performance ensures we are using a reliable unconditional model for motif-scaffolding.
We evaluate the unconditionally trained FrameFlow model by sampling 100 samples from lengths 70, 100, 200, and 300 as done in RFdiffusion.
The results are shown in \cref{table:uncond}.
We find that FrameFlow achieves slightly worse designability while achieving improved diversity and novelty.
We conclude that FrameFlow is able to achieve strong unconditional backbone generation results that are on par with a current state-of-the-art unconditional diffusion model RFdiffusion.
\begin{table}[h]
    \caption{Unconditional generation metrics.}
    \label{table:uncond}
    \begin{center}
        \begin{tabular}{l|ccc}
        \toprule
        \bf Method & \bf Des.($\uparrow$) & \multicolumn{1}{c}{\bf Div. ($\uparrow$)} & \multicolumn{1}{c}{\bf Nov. ($\downarrow$)}
        \\ \midrule
        FrameFlow & 0.86 & 155 & \textbf{0.61} \\
        RFdiffusion & \textbf{0.89} & \textbf{159} & 0.65 \\
        \bottomrule
        \end{tabular}
    \end{center}
\end{table}





% \begin{table}[h]
%   \centering
%   \caption{Forward and inverse folding results.}
%   \begin{tabular}{l|c|c}
%     \toprule
%      & Inverse folding & Forward folding \\
%     Method & scRMSD ($\downarrow$) & RMSD ($\downarrow$) \\
%     \midrule
%     ProteinMPNN & 1.9 $\pm$ 2.7 & N/A \\
%     ESMFold & N/A  & 2.7 $\pm$ 3.9 \\
%     Cogen & 2.2 $\pm$ 2.6 & 15.3 $\pm$ 4.5\\
%     \bottomrule
%   \end{tabular}
%   \label{tab:sampling}
% \end{table}

==> content/method/scaffolding_formulation.tex <==

The full protein backbone is given by $\backbone = [T_1, T_2,\dots,T_N] \in \SE^N$.
The $N$ residues can be separated into the motif $\motif = [T_{i_1},\dots,T_{i_k}]$ where $\{i_1,\dots,i_k\} \subset \{1,\dots,N\}$ and the scaffold $\scaffold=[T_{j_1},\dots,T_{j_{N-k}}]$ is all the remaining residues.
The goal is to model the conditional distribution $p(\scaffold | \motif)$ such that given a motif we can sample diverse scaffolds that pass the designability test in evaluation.
We describe two ways to sample from this distribution with flow matching models.

